Understanding the Role of Input Token Characters in Language Models: How Does Information Loss Affect Performance?

Understanding how and what pre-trained language models (PLMs) learn about language is an open challenge in natural language processing. Previous work has focused on identifying whether they capture semantic and syntactic information, and how the data or the pre-training objective affects their performance. However, to the best of our knowledge, no previous work has specifically examined how information loss in input token characters affects the performance of PLMs. In this study, we address this gap by pre-training language models using small subsets of characters from individual tokens. Surprisingly, we find that pre-training even under extreme settings, i.e. using only one character of each token, the performance retention in standard NLU benchmarks and probing tasks compared to full-token models is high. For instance, a model pre-trained only on single first characters from tokens achieves performance retention of approximately $90$\% and $77$\% of the full-token model in SuperGLUE and GLUE tasks, respectively.

==> ToDo.tex <==
- perplexity
- vowels and consonants models
- improving the analysis
- Rerun superglue on all tasks! Talk with Huiyin/Miles
- Try larger model, e.g. BERT-Large
- GPT pre-training
- See corpus-based metrics for information loss (K)

K:
- I checked the paper "Understanding Dataset Difficulty with V-Usable Information" (\url{https://arxiv.org/pdf/2110.08420.pdf}) and their code (\url{https://github.com/kawine/dataset_difficulty}) but I don't think it can help us because we want to compare training corpora, while their metric is to compare datasets with labels. Need to go with something else.
- For motivation of approaches maybe we can mention something like this viral bionic reading thing (backed by peer reviews studies obviously) (\url{https://lithub.com/will-this-bionic-font-help-you-read-faster/})

Yes we just need standard approaches from Jurafsky and Martin or Manning and Schutze

{
    "ignore": 1705399500,
    "8": 118052972,
    "1": 105471217,
    "2": 335409597,
    "3": 421064347,
    "6": 191530976,
    "5": 233216838,
    "10": 105834677,
    "7": 165943225,
    "4": 313579687,
    "9": 74622488
}


==> reviews_acl.tex <==
============================================================================ 
ACL 2023 Reviews for Submission #3076
============================================================================ 

Title: How much information do large language models actually need from the input tokens?
Authors: Ahmed Alajrami and Nikolaos Aletras
============================================================================
                            META-REVIEW
============================================================================ 

Comments: The reviewers raised concerns on basically every aspect of this work, from the motivation of the research to the methods to the implication of this research. After reading the paper and the comments, I do think revising the paper with these comments will make it stronger.

============================================================================
                            REVIEWER #1
============================================================================

What is this paper about and what contributions does it make?
---------------------------------------------------------------------------
This paper investigates how much information Large Language Models(LLM) need from tokens. This work demonstrates 1)the learning difference between humans and LLM. 2)LLM can retain effective learning when taking a character subset of tokens as input. 3)some certain types of input character subsets achieve better performance than others.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
A. This paper can be interesting to the large language model community.
B. Sufficient experiment results across several datasets have been provided.
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
A. I am not sure if the model has real-world use due to the way of character subset training.
---------------------------------------------------------------------------


Questions for the Author(s)
---------------------------------------------------------------------------
Question A: It seems that the subset vocab doesn't contain full tokens from table 2 and line 284, so how does the LLM predict the full token based on the character subset? (e.g., predict token "half" from the example "ma is ab () th si of ea" in table 1)

Question B: Have you tried to use both two pre-training tasks?

Question C: May you explain why some results approximate random choice( < 50.0) in the SuperGLUE task (e.g., COPA)?
---------------------------------------------------------------------------


Missing References
---------------------------------------------------------------------------
None.
---------------------------------------------------------------------------


Typos, Grammar, Style, and Presentation Improvements
---------------------------------------------------------------------------
It's better to show some cases for the presented model instead of some analysis of different types of input character subsets.
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                               Soundness: 3
                 Excitement (Long paper): 2.5
                     Reviewer Confidence: 4
     Recommendation for Best Paper Award: No
                         Reproducibility: 4
                        Ethical Concerns: No


============================================================================
                            REVIEWER #2
============================================================================

What is this paper about and what contributions does it make?
---------------------------------------------------------------------------
This work performs ablations to the information from individual tokens used by language models. Specifically, the authors keep only one, two, or three characters from each word in a sequence during the pretraining and training processes. They observe an interesting finding that the ablated models do not suffer from a significant performance drop, as measured on downstream tasks/dataset like GLUE and SuperGLUE. They conclude that language models can find patterns in human-unintelligible data. 


However, there are a few concerns that some readers might raise and complain:


(1) Measure of information. The main approach of this work is to explore "the amount of information that LLMs actually need from each individual token" (line 61). However, the amount of information lacks a quantitative definition. Retaining one/two/three characters is a relatively unintuitive measure. Table 2 makes an attempt to give the corresponding vocab size, but we still don't know how much "information" is lost through the ablation process. A potential step can be measuring the entropy of unigrams before and after the character ablation. For the case of retaining three characters, it is possible that not much information is discarded. Moreover, transformers are not unigram, bag-of-words models. Bi-grams and tri-grams (and even n-grams) entropy should be measured on top of the unigram entropy, to support the authors' point that the data is "random" and "limited" (line 568). I.e., a *sequence* of first characters of words may be unique to the corresponding *sequence* of !
 the full words, making the underlying representation not "random".


(2) The authors imply that the ablated models still have satisfactory performance. While this may be true in some probing tasks as shown in Table 5 (with deviation numbers), it is arguable in cases shown in Table 3 (GLUE). Retaining one character for a word results in ~60 avg. GLUE score compared to the original ~80. The determination of whether a reduced performance is still satisfactory is unclear.


(3) The motivation and takeaway of this work is rather vague. The main argument of this work is that language models can effectively find patterns in "seemingly random or limited data", in ways that are "fundamentally different from human cognition" (line 572). However, this is a vague statement, as the language models process "token ids" in practice and even the full words' ids can seem random and unintelligible to humans. It is also relatively unknown how this problem is useful or what insights it gives for future language model designs.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
The paper investigates an interesting problem of ablating the information of individual words being passed into language models. The writing is very clear. The experiments were performed on a comprehensive set of tasks/data.
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
Please see my concerns mentioned above, on a lack of measure for information, an unclear interpretation of results/effectiveness, and a vague motivation and takeaway.
---------------------------------------------------------------------------


Questions for the Author(s)
---------------------------------------------------------------------------
Question A: Have you thought about adding some baseline experiments running on regular subword-based language models, but with a range of different mask rates. Would that be comparable to retaining one/two/three characters for words, but at a sequence level?

Question B:

Question C:
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                               Soundness: 3
                 Excitement (Long paper): 3
                     Reviewer Confidence: 5
     Recommendation for Best Paper Award: No
                         Reproducibility: 3
                        Ethical Concerns: No


============================================================================
                            REVIEWER #3
============================================================================

What is this paper about and what contributions does it make?
---------------------------------------------------------------------------
The paper contributes to answering the question of what large language models (LLMs) actually learn. Prior work has found that LLMs can perform well even with permutated inputs. So, what linguistic processing are LLMs doing?

This paper takes inspiration from cognitive science theory that found that humans can understand a sentence and identify the words from just a few characters, with the rest of the characters omitted. And different position of characters are easier to understand (first, middle, or last character). The authors experiment with LLMs pre-trained and fine-tuned using a modified corpus, where each token (word) is replaced by a subset of its characters of length 1, 2, or 3. 

Results indicate that different parts of the input contribute differently towards learning. In particular, the first character is the most informative, followed by the last character, or a combination of the first and last characters. Furthermore, models trained using a subset of characters still learn comparable linguistic capabilities to the models trained on the full tokens, according to probing tasks.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
The paper performs a wide range of insightful experiments. It does a good job explaining the results. It does not provide a deep explanation on the consequences of these findings or the reason behind them. However, I expect this paper to be of interest to the community. The connections to cognitive science are very interesting.
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
- The paper does great experimental work. However, there is no analysis or discussion of the implications of those findings towards LLM understanding, or how it would be of use.

- It is very intriguing that the performance of models with minimal characters is higher than the full token input in some SuperGLUE tasks. There is no mention or discussion of this in the text.

- The authors credit the work of Krishna et al. (2021) for the finding that a transformer trained with random character n-grams can perform comparably well to standard models. Then, the contributions of this paper are limited to the finding that different choices for those random characters can be more informative.
---------------------------------------------------------------------------


Questions for the Author(s)
---------------------------------------------------------------------------
Question A: Why it is useful to evaluate your approach on SuperGLUE in addition to GLUE? What different conclusions can we make from that experiment?
---------------------------------------------------------------------------


Typos, Grammar, Style, and Presentation Improvements
---------------------------------------------------------------------------
L264 "we concatenate sentences to make sure the total number of tokens is under 512.": I don't think this is correct. How does concatenation contribute to the sentence being shorter than 512 tokens?
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                               Soundness: 4
                 Excitement (Long paper): 3.5
                     Reviewer Confidence: 3
     Recommendation for Best Paper Award: No
                         Reproducibility: 5
                        Ethical Concerns: No


============================================================================
                            REVIEWER #4
============================================================================

What is this paper about and what contributions does it make?
---------------------------------------------------------------------------
The paper studies the performance degradation of large language models when they are trained only on a subset of characters for each word. The models trained on 1/2/3 characters are evaluated on different NLU benchmarks and probing tasks and they are compared to models trained on complete tokens. The authors show that the performance is lower when we use only a limited number of characters, but it is still clearly above chance.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
The experimental setup is robust, going through a wide range of tasks. Also, the dataset adaptation is sound and it covers different input ablations.
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
I consider that the motivation and the impact of the paper are unclear. I think it requires a deeper connection to the phenomena the authors investigate, either from a cognitive science or psycholinguistics perspective.

Second, one of the main contributions of the paper doesn't seem to be completely met. In order to claim that the paper sheds light on the differences between LLMs and human reading comprehension, the authors would need more evidence, coming from a comparison between human and LLM behaviour.

Even though the analysis covers a wide range of tasks, I think it would be valuable to understand how other variables impact the model performance, like the proportion on characters that are discarded or the ambiguity level brought by keeping only a specific set of characters. For example, Figure 1 shows that a big proportion of tokens have 2-3 characters, so these tokens wouldn't suffer any alteration in the modified datasets. 

Also, a deeper understanding of why and where the model fails/succeeds in the case of the probing tasks is important for a complete understanding of the input ablation impact. This can be achieved through some qualitative analysis or strong linguistic arguments that would justify it. For example, some semantic tasks would have clear patterns that can be associated with the last characters of the words (Tense, SubjNumb, ObjNum). Finally, adding some baselines for the probing tasks (random label or most frequent class) would bring more context to the results. For instance, in the case of ObjNum, the model achieves 58% with some input input ablation setups, which is very low for a binary classification task.
---------------------------------------------------------------------------


Questions for the Author(s)
---------------------------------------------------------------------------
Question A: Do you think that these findings would be similar on models on different sizes ?

Question B: How does the information in Table 2 compare with the full token model ?

Question C: Does the input ablation have any impact on the speed or the memory usage of the models ? Is the training more efficient in the proposed setup ?
---------------------------------------------------------------------------


Missing References
---------------------------------------------------------------------------
Considering that the study is inspired by cognitive science and psycholinguistics research on orthographic priming, I would recommend to give more context to this literature and how the current work is connected to it in the "Related Work" section.
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                               Soundness: 3
                 Excitement (Long paper): 2.5
                     Reviewer Confidence: 4
     Recommendation for Best Paper Award: No
                         Reproducibility: 4
                        Ethical Concerns: No


